Progressive Reinforcement Learning with Distillation for Multi-Skilled Motion Control

Deep reinforcement learning has demonstrated increasing capabilities for continuous control problems, including agents that can move with skill and agility through their environment. An open problem in this setting is that of developing good strategies for integrating or merging policies for multiple skills, where each individual skill is a specialist in a specific skill and its associated state distribution. We extend policy distillation methods to the continuous action setting and leverage this technique to combine expert policies, as evaluated in the domain of simulated bipedal locomotion across different classes of terrain. We also introduce an input injection method for augmenting an existing policy network to exploit new input features. Lastly, our method uses transfer learning to assist in the efficient acquisition of new skills. The combination of these methods allows a policy to be incrementally augmented with new skills. We compare our progressive learning and integration via distillation (PLAID) method against three alternative baselines.

==> tex/acknowledgments.tex <==
\section{Acknowledgements}

==> tex/old_results.tex <==
\section{Experiments}

The method in this work is evaluated on a humanoid robotic simulation.
% The first environment is similar to the one used in~\cite{2016-TOG-terrainDeepRL}.
Here a bipedal character is trained to navigate multiple types of terrain, including \gaps and \steps, shown in~\refFigure{fig:distilatibon-environemnts-gap} and \refFigure{fig:distilation-environemnts-stairs}.
The environment used is similar to the environments used in~\cite{PengP16} where the goal is to find the proper joint torques to establish a robust walking gait.
We add additional terrain types to this problem as well.
An example of a biped trained to walk on an \incline is shown in~\refFigure{fig:distilation-environemnts-incline}.

\begin{figure}[h!]
\subcaptionbox{\label{fig:2D-LLC-gap}}{ \includegraphics[width=0.3\columnwidth]{images/sim/biped_FSM_gap}}
\subcaptionbox{\label{fig:2D-LLC-stairs}}{ \includegraphics[width=0.3\columnwidth]{images/sim/biped_FSM_stairs.png}}
\subcaptionbox{\label{fig:2D-LLC-incline}}{ \includegraphics[width=0.3\columnwidth]{images/sim/genBiped_slope}} \\
\caption{
\todo{Three different environments are used to evaluate this work.
The first two use a \FSM to control the overall \character gait cycle.
This \FSM is parameterized and trained to navigate multiple types of terrain.}
In the last environment a biped (\pdcontrollerText), controlled by specifying pd joint targets at \valueWithUnits{$30$}{Hz}, learns to walk up a random \incline.
}
\label{fig:2D-LLC-environemnts}
\end{figure}

\subsection{Distillation}

Distillation is used to combine expert policies, allowing for efficient training of a new policy with the capabilities of both experts.

\subsubsection{FSM}
We start by training an \FSM \agent to run across flat terrain.

In \refFigure{fig:distilation-evalution-compare} is a comparison between a \FSM that has been distilled on \gaps, and \walls and is now learning to navigate \slopes.
This is compared to the \MultiTasker that attempts to learn all skills at once. 
The \MultiTasker has a challenging time learning learning all skills at one.
The \DistilRLer uses the transfered skills to learn the new skill faster than the \MultiTasker.

We investigate this property further in~\refFigure{fig:distilation-evalution-multiple-policies} were we train a randomly initialized policy on \steps and another that trains on \steps and \gaps. 
Here we compare just the iterations spent learning the \steps task, where the \MultiTasker will have seen half the number as the \expert.
Still the \MultiTasker learns the skill faster than the \expert.
\todo{There is a similar argument found in distrl}


\subsubsection{LLC}


\todo{Some nice way of displaying the chain:}
\glen{I am not sure the readers are going to be overly interested in the particular details of the tasks we are combining or there sequence.}


01 flat \\

02 transf from 1 hard\_ramp, scratch \\
03 distill 1, 2 
	(terrain inject 1) \\

04 transf from 2 easy\_steps, scratch - baseline 
	(terrain inject 2) \\
05 transf from 3 easy\_steps - distill \\
06 distill 3, 5 \\

07 transf from 4 rough\_slopes, scratch - baseline \\
08 transf from 6 rough\_slopes - distill \\
09 distill 6, 8 \\

In this experiment, our set of tasks consists of 5 different terrains that a 2D humanoid walker must traverse. The details of the learning tasks as well as the reinforcement learning algorithm closely follow those outlined in \cite{PengP16}. The goal in these tasks is to maintain a consistent forward velocity traversing various terrains while also trying to match a supplied motion capture clip of a natural human walking gait on flat ground. The 2D humanoid receives as input both a character and terrain state representation. A detailed description of the experimental setup is included in \todo{Appendix A}.
The tasks are presented to the continual learner sequentially and the goal is to progressively learn to traverse all of the terrain types.

We evaluate our approach against two baselines. Firstly, to demonstrate that knowledge from previous tasks can be effectively transferred after integration steps, we compare the learning progress from learning new tasks in our framework with learning them from scratch. Second, we demonstrate that iterated \distillationText is effective for retention of learned skills. 
% by comparing the policy performance on all previous tasks after each task integration step to the respective \expert for that policy and a baseline.

\begin{figure}[!ht]
\centering 

\subcaptionbox{\label{fig:distilation-environemnts-flat}}{ \includegraphics[width=0.32\columnwidth]{images/terrain/flat.png}}
\subcaptionbox{\label{fig:distilation-environemnts-incline}}{ \includegraphics[width=0.32\columnwidth]{images/terrain/ramp.png}}
\subcaptionbox{\label{fig:distilation-environemnts-steps}}{ \includegraphics[width=0.32\columnwidth]{images/terrain/steps.png}} \\
\caption{
Three of the environments being used to evaluate this work.
% The first two use a \FSM to control the gait cycle.
% This \FSM is parameterized and trained to navigate \gaps and \steps.
(a) \pdcontrollerText walking on \Flat terrain.
(b) \pdcontrollerText walking on \incline terrain.
In the last environment, the \pdcontrollerText, is controlled by specifying joint targets at \valueWithUnits{$30$}{Hz}, learns to walk up a random \incline.
\todo{These should be zoomed in more, I can hardly make out the \character}
}
\label{fig:distilation-environemnts}
\end{figure}

\paragraph{Transfer Learning}

Here the \pdcontrollerText is trained to produce a walking motion on flat ground. 
We then initialize training on a similar task with slanted ground at random inclines (this task type is labelled \incline), and compare it to training a controller from scratch on the inclined ground task.
We show in~\refFigure{fig:transfer_2DLLC-gap} the large benefit from using transfer learning for this problem.
Even though the \TL controller and the from scratch controller begin with about the same average reward the \TL accelerates the learning process.

\begin{figure}[!ht]
\subcaptionbox{\label{fig:transfer_2DLLC-gap}}{ \includegraphics[width=0.3\columnwidth]{images/transferLearning/compare_reward_llc_ramp.pdf}}
\subcaptionbox{\label{fig:transfer_2DLLC-stairs}}{ \includegraphics[width=0.3\columnwidth]{images/terrain/ramp.png}}
\subcaptionbox{\label{fig:transfer_2DLLC-distilation}}{ \includegraphics[width=0.3\columnwidth]{images/transferLearning/distill_flat_ramp_transfer_to_slopes}}
\caption{(a) \pdcontrollerText walking on \Flat terrain.
(b) \pdcontrollerText walking on \incline terrain.
\todo{(b) is the same as \refFigure{fig:distilation-environemnts-incline}}
(c) The result of learning the task of walking on slopes starting with a policy that distilled the skills of walking on flat and inclined ground \todo{What do the three plots mean in (c)? I think we only want to show the bottom plot.} \glen{Was this also TL on flat+slopes?}.
}
\label{fig:transfer_2DLLC}
\end{figure}

The \FromScratch version is trained to learn the task from a randomly initialized policy. The \DistilRLer version initializes its policy with one that was trained to walk on flat ground. The \MultiTasker version is also initialized its policy from one trained to walk on flat ground but also alternates between \Flat and \incline during training. 
The \MultiTasker version is designed to evaluate the affects of adding skills to an \agent while training on the old skills to prevent forgetting.
This is in contrast to using a distillation method that will integrate skills together after each new skill is learned. \glen{The problem with the \MultiTasker is that the controller is making policy improvement choices with respect to the reward. In the worst case a particular task could have very high reward and receive unfair priority over other tasks.}
\todo{Might be good to outline the three different methods somewhere, with their strengths and weaknesses.}

In~\refFigure{fig:distilation-evalution-gaps} the \DistilRLer is compared to the two baselines for this work.
The \FromScratch method learns the slowest as it is given no information about how to perform similar skills.
The \MultiTasker method is initialized from a controller that was train to walk on flat ground. 
This controller has to learn multiple tasks together, this complicates the learning progress as simulation for each tasks is split across the training process.
This is in contrast to using a distillation method that will integrate skills together after each new skill is learned.
However, it has been shown that training across many tasks at once can increase overall learning speed and potentially reduce forgetting~\todocite{}\todo{If the tasks share a similar reward function.}\glen{Also shown in~\refFigure{fig:distilation-evalution-multiple-policies}}. 
This is also shown in 
The \DistilRLer method is trained for only learning to walk up an \incline.
This allows the training to quickly learn by focusing on a single task and gain the benefits of transferring knowledge related to walking on \Flat ground.

\begin{figure}[ht!]
\centering
\subcaptionbox{\label{fig:distilation-evalution-compare}}{ \includegraphics[width=0.32\columnwidth]{images/distilation/learning_speed_comp_between_distill_on_slopes_and_baseline_random_init}}
\subcaptionbox{\label{fig:distilation-evalution-multiple-policies}}{ \includegraphics[width=0.32\columnwidth]{images/distilation/DistExpVsMultGaps}}
\subcaptionbox{\label{fig:distilation-evalution-gaps}}{ \includegraphics[width=0.32\columnwidth]{images/distilation/learning_speed_comp_between_tl_from_flat_to_ramp}}
\caption{
(a) A comparison between a policy that learns to walk on \incline transfer learning from a policy that learned \Flat compared to a policy learning from scratch.
Blue is the \DistilRLer and orange is the \FromScratch method.
(b) Shows that the \MultiTasker can learn faster training on \steps and \gaps than an \agent learning the single task \steps does.
(c) Shows the benefit of using distillation when learning a new task/skill, \incline, when the controller has some knowledge of \Flat.
% The \emph{Scratch} version is trained to learn the task from a randomly initialized policy. 
The \DistilRLer initializes its policy with one that was trained on \Flat. The \MultiTasker is also initialized from a policy trained on \Flat but also alternates between \Flat and \incline during training. 
% The \MultiTasker is designed to evaluate the affects of adding skills to an \agent while training on the old skills to prevent forgetting.
\todo{Need policy evaluation comparison for with and without DAGGER.}
}
\label{fig:distilation-evalution}
\end{figure}

These results show the the \MultiTasker can have comparable performance to the \DistilRLer on tasks with similar rewards. Next, we investigate how these methods compare as more types of tasks are added.

\paragraph{Distilling Multiple Policies}
\todo{Distillation can benefit from learning multiple tasks at the same time} see Figure~\ref{fig:distilation-evalution-multiple-policies}

\todo{Distilling more policies can also make it difficult to do well on any particular policy}

Learning multiple tasks at the same time my help the \agent learn tasks quicker but this method may not scale with respect to the number of tasks.
When training the \MultiTasker over two or even three tasks (\refFigure{fig:distilation-multitask-3}) the method shows improvement, however when learning a fourth task the method appears to struggle~\refFigure{fig:distilation-multitask-4}.
Using distillation to combine the skills of many policies appears to scale better with respect to the number of skills being integrated.
This is likely because distillation is a semi-supervised method which is more stable than the un-supervised RL problem. 
This can be seen in~\refFigure{fig:distilation-distiller-3} and \ref{fig:distilation-distiller-4} where the \DistilRLer combines the skills faster, and can find \todo{higher value policies in practice}.


\begin{figure}[ht!]
\centering
\subcaptionbox{\label{fig:distilation-multitask-3}}{ \includegraphics[width=0.48\columnwidth]{images/distilation/multi_reward_across_flat_ramp_steps}}
\subcaptionbox{\label{fig:distilation-distiller-3}}{ \includegraphics[width=0.48\columnwidth]{images/distilation/005startdistill_reward_distilling_flat_incline_steps_into_one}}
\subcaptionbox{\label{fig:distilation-multitask-4}}{ \includegraphics[width=0.48\columnwidth]{images/distilation/multitasker_reward_over_4_tasks}}
\subcaptionbox{\label{fig:distilation-distiller-4}}{ \includegraphics[width=0.48\columnwidth]{images/distilation/007startdistill_reward_distilling_flat_incline_steps__slopes_into_one}}
\caption{
These figures show the average reward a particular policy achieves over a number of tasks.
After learning an \expert for \Flat + \incline a new \steps task is trained. Figure (a) shows the performance for the \MultiTasker and figure (b) for the \DistilRLer.
The \DistilRLer learns the combined tasks fast, however the \MultiTasker achieves marginally better average reward over the tasks
Figures (c,d) show the performance of an \expert on \Flat + \incline + \steps trained to learn the new task \slopes for the \MultiTasker (c) and \DistilRLer (d).
After including another task (\slopes) the \MultiTasker struggles to achieve its previous performance and the \DistilRLer combines the tasks gracefully.
 \cheng{Interesting to note that the \MultiTasker is starting to hit its limits.}
\todo{Need to fix slopes for \ref{fig:distilation-multitask-4}, maybe cut he x-axis to 300,000}
 }
\label{fig:distilation-evalution-multitasker}
\end{figure}

% \subsection{Terrain RL Environment}

\paragraph{Terrain Types}
\todo{Need Videos and images for each terrain type, \gaps, \steps, \slopes and \Flat.}

\paragraph{Transfer Learning}
Given the many types of tasks learning can be done more efficiently by using transfer learning. First, a controller can be trained on \gaps then transfered to \steps.
Where parts of the policy that, for example, identify upcoming obstacles, can be used across multiple skills.

\begin{figure}[!ht]
\centering
\subcaptionbox{\label{fig:FSM-transfer-gaps-stairs}}{ \includegraphics[width=0.3\columnwidth]{images/transferLearning/DistScratchVsTransfMixed}}
\subcaptionbox{\label{fig:FSM-transfer-walls-gaps}}{ \includegraphics[width=0.3\columnwidth]{images/transferLearning/DistScratchVsTransfMixed}}
\caption{ 
Comparison of the helpfulness  of transfer learning over a couple of different environment pairs (gaps-> stairs, walls -> gaps, cliffs -> gaps)
\todo{Perform these other comparisons}
}
\label{fig:FSM-evalution}
\end{figure}

\paragraph{Discussion}
Distillation seems to work very well for this particular problem. 
However, our evaluation shows that there is no significant gains when transfer learning between tasks.
We believe this is because of the robustness built into the FSM controller. 
\todo{This robustness increases the \emph{basin of attraction} for the controller making it easier to learn a good policy.}
\glen{This means to really benefit from TL the tasks not only need to be similar but also need to be challenging.}

\todo{A paragraph on forgetting}

\subsection{Feature Injection}

\todo{Terrain Injection Stuff}
An appealing property of the distillation approach is that the combined policy model need not resemble that of the individual expert controllers. Two different experts lacking state features (in this case terrain) and trained with invariable terrain can be combined into a single policy that has new state features for the terrain in order to differentiate these tasks. 
In our framework we wish to initialize the aggregation step with the previous policy. 
We introduce the idea of \emph{feature injection} for this purpose. 
We augment a policy with additional features while allowing it to retain its original functional behaviour in a way similar to \cite{chen2015net2net}.
This is achieved by adding additional inputs to the neural network and initializing the weights and biases associated with these new features to 0. 
this approach is demonstrated in the third step of the experiment by combining the blind \Flat and \incline \expert policies via distillation.
\todo{Maybe run an experiment to compare if the way we do terrain injection is better than random initialization (definitely helps with direct transfer, but what about for distill?)}

\begin{figure}[!ht]
\subcaptionbox{\label{fig:transfer-eval_2DLLC-gap}}{ \includegraphics[width=0.3\columnwidth]{images/transferLearning/CleanDistill004v005.png}}
\subcaptionbox{\label{fig:transfer-eval_2DLLC-stairs}}{ \includegraphics[width=0.3\columnwidth]{images/terrain/steps.png}}
\caption{
}
\label{fig:transfer-eval_2DLLC}
\end{figure}


